Latent Space Inference For Spatial Transcriptomics

In order to understand the complexities of cellular biology, researchers are interested in two important metrics: the genetic expression information of cells and their spatial coordinates within a tissue sample. However, state-of-the art methods, namely single-cell RNA sequencing and image based spatial transcriptomics can only recover a subset of this information, either full genetic expression with loss of spatial information, or spatial information with loss of resolution in sequencing data. In this project, we investigate a probabilistic machine learning method to obtain the full genetic expression information for tissues samples while also preserving their spatial coordinates. This is done through mapping both datasets to a joint latent space representation with the use of variational machine learning methods. From here, the full genetic and spatial information can be decoded and to give us greater insights on the understanding of cellular processes and pathways.

==> PackagesLoadedbyTemplate.tex <==
% University of Pennsylvania Ph.D. Dissertation LaTeX Template packages

upennstyle.sty loads the following packages
\begin{itemize}
\item geometry 
\item fontenc
\item babel
\item csquotes
\item amsthm
\item amsmath
\item amssymb
\item amsfonts
\item amscd
\item calc
\item graphicx
\item float
\item caption
\item multirow
\item blindtext
\item verbatim
\item parskip
\item titlesec
\item appendix
\item setspace
\item array
\item tabularx
\item booktabs
\item pdflscape
\item hyperref
\item tocloft
\end{itemize}

sampledissertation.tex loads the following packages
\begin{itemize}
\item upennstyle
\item natbib
\end{itemize}
